Agent World Model in the Wild: Computer-Use Agent Environment Synthesis

Agent learning is shifting from learning from human data toward learning through interaction with the world. However, scaling such learning directly in real-world computer systems is challenging and can introduce substantial security risks. We therefore propose Agent World Model in the Wild (WildAWM), a scalable pipeline for synthesizing controllable environments and tasks for training general computer-use agents (CUAs). Whereas existing approaches typically specialize in a single agent interaction interface, we construct executable environments that jointly support graphical user interfaces, model context protocol services, and command-line interfaces, allowing agents to flexibly combine visual interaction, tool use, and code execution. WildAWM is entirely powered by open-source models, demonstrating that high-quality computer-use environments can be generated without proprietary frontier models. Beyond environments, we address three recurring challenges in task synthesis: ensuring solvability, maintaining sufficient difficulty, and producing reliable verifiers, by introducing execution-based quality gates that combine heterogeneous agent rollouts, cross-judge consistency checks, and counterfactual probes of judgment robustness. The resulting pipeline synthesizes 341 long-horizon environment-task pairs that can require over 100 agent steps to solve and remain challenging even for frontier models, with GPT-6-Astra solving only 60% of them. We train two Qwen models of different sizes exclusively in these synthetic worlds. Both models achieve substantial gains across 8 out-of-distribution benchmarks spanning web, claw, and computer-use agents, demonstrating that learning in WildAWM's synthesized worlds generalizes broadly to unseen computer-use tasks. The code is publicly available at https://github.com/MSR-Orchard/WildAWM.

==> paragraph_refs.tex <==
\makeatletter
\newcommand*{\myparagraph@parentnumber}{%
  \ifnum\value{subsubsection}>0
    \thesubsubsection
  \else\ifnum\value{subsection}>0
    \thesubsection
  \else
    \thesection
  \fi\fi
}
\NewDocumentCommand{\myparagraph}{O{} o m}{%
  \expandafter\ifx\expandafter\relax\detokenize{#1}\relax
  \else
    \begingroup
      \let\myparagraph@savedhref\@currentHref
      \phantomsection
      \edef\@currentlabel{\myparagraph@parentnumber}%
      \IfNoValueTF{#2}{\GetTitleString{#3}}{\GetTitleString{#2}}%
      \let\@currentlabelname\GetTitleStringResult
      \label{#1}%
      \global\let\@currentHref\myparagraph@savedhref
    \endgroup
  \fi
  \paragraph{#3}%
}
\makeatother

\NewDocumentCommand{\parref}{O{Sec.} m}{%
  \hyperref[#2]{#1~\ref*{#2} (\nameref*{#2})}%
}

